Probing the Kinematics of Multiple- and Single-Protostar Systems in Perseus with N2H+

We analyze the dense gas kinematics in two Class 0/I protostellar cores, Per 30 and NGC 1333 IRAS 7, in the Perseus molecular cloud to determine whether their velocity structures are indicative of rotation. We examine the hyperfine structure of the N2H+ J=1-0 transition by combining 3" (900 AU) Atacama Large Millimeter/Submillimeter Array (ALMA) measurements with 9" (2700 AU) measurements from the Green Bank Telescope (GBT). We use the CASA Feather method to combine these data in order to maximize our sensitivity across spatial scales. We fit the N2H+ spectra to constrain the centroid velocity of the gas at each pixel and use these values to calculate the linear velocity gradient and specific angular momentum within apertures centered on each protostar with radii ranging from 5-60". Our results indicate that the velocity structure probed by the N2H+ emission is likely not a result of core rotation. These findings are consistent with other studies in the literature which indicate rotation is often not evident on scales less than 1000 AU. We instead suggest that the velocity structure we see is a result of torques caused by irregular density distributions in these protostellar systems.

==> Notes.tex <==
%Per\,18's outflow runs nearly north-south, with a position angle of 345 degrees, while its near neighbor Per\,21, separated from Per\,18 by $\sim2500$\,AU has an outflow with a position angle of 48 degrees \citep{Tobin2016}. Per\,49, which is 


%\begin{itemize}
%    \item introduce sources (evolutionary state, outflows, known disc, distances between sources)
%    \begin{itemize}
%        \item NGC 1333 IRAS\,7
%        \begin{itemize}
%            \item quintuple system--both Per\,18 and Per\,49 have companions that are separated by less than 100 AU \citep{Tobin2016}--Per\,18 binary separation $\sim25$\,AU \citep{Reynolds2024}
%            \item Per\,18 and Per\,21 are Class 0 sources, while Per\,49 is Class I
%            \item Per\,18 shows evidence for disk fragmentation as a result of gravitational instability \citep{Tobin2016}--dust continuum knot present on eastern side of protostar--need evidence of rotationally-supported disk
%            \item \cite{Reynolds2024} resolves disks of Per\,21 and Per\,18 binary
%            \begin{itemize}
%                \item Per\,18 disks (likely formed via disk fragmentation): A (eastern): PA $\sim73$\,deg, incl $\sim65$\,deg; B: PA $\sim80$\,deg, incl $\sim77$\,deg
%                \item Per\,21 disk: PA $\sim74$\,deg, incl $\sim16$\,deg
 %               \item Per\,49 disks: not studied by \cite{Reynolds2024}, but \cite{Tychoniec2020} found that the two disks that make up Per\,49 have sizes of about 0.18$^{\prime\prime}$ and 0.38$^{\prime\prime}$ and \cite{Tobin2018} reports separation of $\sim0.3^{\prime\prime}$ ($\sim94$\,AU)
  %          \end{itemize}
   %         \item Per\,18 has outflow with PA = 345 deg \citep{Tobin2016}
    %        \begin{itemize}
     %           \item redshifted outflow--150 deg \citep{Stephens2017}
      %          \item blueshifted outflow-- -30 deg \citep{Stephens2017}
       %         \item \cite{Tobin2018} detect $^{13}$CO, C$^{18}$O, SO, and H$_{2}$CO toward Per\,18, which all trace velocity gradients perpendicular to outflow direction--\cite{Tobin2018} interpret this as support for kinematics being accounted for by rotation
        %    \end{itemize}
        %    \item Per\,21 has outflow with PA = 48 deg \citep{Tobin2016}
        %    \item Per\,49 has outflow with PA = 27 deg \citep{Stephens2017}
        %\end{itemize}
        %\item Per\,30
        %\begin{itemize}
        %    \item isolated protostar
        %\end{itemize}
    %\end{itemize}
%\end{itemize}

